Towards Relating Ciao Assertions and LPTP Theorems

Abstract interpretation-based verification is a central component of the Ciao Prolog system, enabling expressive specifications of properties of programs, predicates, and execution states. Independently, the LPTP (Logic Programming Theorem Proving) framework offers a first-order logical formalism for expressing and proving properties of predicates. In this paper, we address a fundamental issue in relating these two frameworks: studying the translation of Ciao assertions into LPTP formulae and identifying a partial correspondence between assertion-based and logic-based specifications. We introduce a systematic translation scheme, characterize assertion classes according to their logical encodability, and propose approximation strategies and auxiliary constructs for non-translatable cases, and finally analyze the resulting soundness and completeness trade-offs. We argue that our proposal enables a tight integration of Ciao's assertion checking with LPTP-based deductive verification, thereby leveraging their complementary capabilities.

==> eptcsdata.tex <==
\providecommand{\firstpage}{223}
\providecommand{\publicationstatus}{W. Faber, L. Giordano, R. Rocha, V. Santos Costa (Eds.):\\ 42nd International Conference on Logic Programming (ICLP 2026)\\
EPTCS 450, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.450.18}{10.4204/EPTCS.450.18}}

